Grounding Representation Similarity with Statistical Testing

To understand neural network behavior, recent works quantitatively compare different networks' learned representations using canonical correlation analysis (CCA), centered kernel alignment (CKA), and other dissimilarity measures. Unfortunately, these widely used measures often disagree on fundamental observations, such as whether deep networks differing only in random initialization learn similar representations. These disagreements raise the question: which, if any, of these dissimilarity measures should we believe? We provide a framework to ground this question through a concrete test: measures should have sensitivity to changes that affect functional behavior, and specificity against changes that do not. We quantify this through a variety of functional behaviors including probing accuracy and robustness to distribution shift, and examine changes such as varying random initialization and deleting principal components. We find that current metrics exhibit different weaknesses, note that a classical baseline performs surprisingly well, and highlight settings where all metrics appear to fail, thus providing a challenge set for further improvement.

==> checklist.tex <==
\section*{Checklist}
\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See Section \ref{section:discussion}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See Section \ref{section:discussion}. }
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{See Section \ref{section:setup}, Section \ref{section:results}, and Appendix \ref{appendix:pretraining} for details to reproduce the experimental results.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Appendix \ref{appendix:pretraining} and \ref{appendix:finetuning} .}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{See Figure \ref{fig:display_variation}, Appendix \ref{appendix:layer-wise-results} and Appendix \ref{appendix:bootstrap}.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Appendix \ref{appendix:pretraining} and \ref{appendix:finetuning}. }
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{See Section \ref{section:setup} and Section \ref{section:results} }
  \item Did you mention the license of the assets?
    \answerYes{See Appendix \ref{appendix:licenses} }
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}


==> table.tex <==
\begin{table}[t]
	\caption{Summary of rank correlation results \js{this needs a bit more info (not clear that (p) means p-value, and also mysterious why it only appears for one of the rows; actually didn't we compute p-values for a couple different rows, or was it really just one?} \js{I'd also say something about what conclusion the reader should draw from the table}}
	\label{table:results}
	\begin{tabular}{@{}cccccccc@{}}
	\toprule
	\multirow{2}{*}{Perturbation}                                                             & \multirow{2}{*}{Functionality}                                  & \multicolumn{2}{c}{Procrustes}                                                                                                          & \multicolumn{2}{c}{CKA}                                                                                             & \multicolumn{2}{c}{PWCCA}                                                                                                             \\ \cmidrule(l){3-8} 
																							  &                                                                         & $\rho$ (p)                                                         & $\tau$ (p)                                                         & $\rho$ (p)                                               & $\tau$ (p)                                               & $\rho$ (p)                                                        & $\tau$ (p)                                                        \\ \midrule
	\multirow{2}{*}{\begin{tabular}[l]{@{}l@{}}Pretraining seed, \\ layer depth\end{tabular}} & QNLI probe                                                              & 0.574                                                              & 0.435                                                              & \textbf{0.628}                                           & \textbf{0.473}                                           & 0.491                                                             & 0.368                                                             \\ \cmidrule(l){2-8} 
																							  & SST-2 probe                                                             & 0.624                                                              & 0.474                                                              & \textbf{0.679}                                           & \textbf{0.512}                                           & 0.556                                                             & 0.42                                                              \\ \midrule
	\begin{tabular}[l]{@{}l@{}}Pretraining seed, \\ PC deletion\end{tabular}      & SST-2 probe                                                             & 0.895                                                              & 0.73                                                               & 0.795                                                    & 0.643                                                    & \textbf{0.918}                                                    & \textbf{0.76}                                                     \\ \midrule
	Finetuning seed                                                                           & \begin{tabular}[c]{@{}c@{}}HANS: Lexical \\ (non-entailed)\end{tabular} & \textbf{\begin{tabular}[c]{@{}c@{}}0.551\\ (4.8e-07)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}0.398\\ (6.1e-07)\end{tabular}} & \begin{tabular}[c]{@{}c@{}}0.462\\ (2.3e-3)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.329\\ (2.6e-3)\end{tabular} & \textbf{\begin{tabular}[c]{@{}c@{}}0.568\\ (1.2e-6)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}0.412\\ (1.8e-6)\end{tabular}} \\ \midrule
	\multirow{2}{*}{\begin{tabular}[l]{@{}l@{}}Pretraining, \\ finetuning seeds\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Antonymy\\ stress test\end{tabular}          & \textbf{0.243}                                                     & \textbf{0.178}                                                     & 0.227                                                    & 0.16                                                     & 0.204                                                             & 0.152                                                             \\ \cmidrule(l){2-8} 
																							  & \begin{tabular}[c]{@{}c@{}}Numerical\\ stress test\end{tabular}         & 0.071                                                              & 0.049                                                              & \textbf{0.122}                                           & \textbf{0.084}                                           & 0.031                                                             & 0.023                                                             \\ \bottomrule
	\end{tabular}
\end{table}

